Heart-Based Biometric Protocols: A look back over almost two decades

This article surveys the literature over the period 2003-2021 on heart-based biometric protocols. In particular, we focus on how the heart signal is transformed from a continuous wave to discrete values to be used afterwards in authentication protocols. We explain and classify the surveyed proposals according to three main parameters: i) the dataset they use for testing their results; ii) the delineation algorithms they use to extract the fiducial points, and; iii) the cryptographic tests they run (if any) to validate how random the extracted token is.

==> sections/analysis.tex <==
\section{Review of Proposed Works}\label{sec:analysis}

%The literature regarding this quantization algorithm is, unfortunately, a bit obscure in the sense that the first authors did not provide a full description of the algorithm. They computed the \glspl*{IPI} and generated tokens of 128 bits by using a coding scheme $I_i(i=0,1)$ \cite{Bao2005}. One of the most known paper in the community was the one proposed by Poon \etal\ \cite{Poon2006}, where the authors quantized the \gls*{ECG} signal and coded the extracted \glspl*{IPI} into 128 bits tokens. Sadly and once again, authors did not provide much more information about how the quantization algorithm is performed. 

%Contrarily to this tendency, in 2013 Rostami \etal\ \cite{Rostami2013} not only the provided more details about how the quantization algorithm they used works but also they shared with us the source coded when requested. In the following, we are explaining in more detail how this algorithm works whereas in \Cref{sec:analysis} we provide detailed information about the contributions done in this area. 

==> sections/applications.tex <==
\section{Heart-Based Cryptographic Protocols: Applications}\label{sec:applications}

\pica{to classify}
In 2010, Venkatasubramanian and Gupta \cite{Venkatasubramanian2010} proposed an \gls*{IPI}-based protocol to secure communications between sensors in a \gls*{BSN}. This protocol was based on Poon \etal 's work \cite{Poon2006} and authors did not corroborate the entropy of \gls*{IPI} values. 





\subsection{Authentication Protocols}\label{subsec:biometric_protocols}
\pica{check Xu2011}
Rostami \etal\ \cite{Rostami2013} in 2013, proposed a security protocol where a patient equipped with an \gls*{IMD} and a doctor with a programmer can extract the same nonce from the patient's \gls*{ECG} and thus mutually authenticate each other. Similar assumptions are made in \cite{Poon2006,Zheng2015,Xu2011}, just to cite a few of them. 

Koya \etal\ \cite{Koya2018} proposed a hybrid mutual authentication and key agreement scheme for \glspl*{WBAN}. Authors appended the four \glspl*{LSB} to create a 128-bits token and tested their proposal against both ptbdb and mitdb databases. Similarly to previous works, authors just calculated the standard Shannon entropy to check and claim that the generated tokens are random.

Ingale \etal\ \cite{Ingale2020} recently published a comparative analysis of \gls*{ECG} biometric authentication protocols. In it, authors compare the most important proposals on authentication protocols, and propose a new authentication mechanism that achieves over 100\% of accuracy. Authors do not provide information enough to replicate their results, \eg\ \gls*{WT} algorithms and bits extracted. In addition to that, they only use 20 patients of cebsdb public databases---which is composed of 60 patients in total, and they do not justify nor detail which ones they use. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Key/Token Generation}\label{subsec:key_distribution}
In 2011 Xu \etal\ \cite{Xu2011} proposed IMDGuard, a security scheme for \glspl*{IMD} where the key establishment is based on \glspl*{IPI}. Authors were the first who introduced the \textit{quantization} algorithm, concluding that the last 4 bits of the \glspl*{IPI} are random by running a subset of \gls*{NIST} tests \cite{Bassham:2010:SRS:2206233}.

Hu \etal\ proposed OPFKA \cite{Hu2013}, a secure key establishment protocol. However, authors:
\begin{inparaenum}[1)]
    \item did not corroborate previous results, and;
    \item did not mention which databases from Physionet repository they used for their experiments.
\end{inparaenum}

Seepers \etal\ \cite{Seepers2017} proposed in 2017 a key generation procedure based on \glspl*{IPI}. Regarding the entropy evaluation, authors analyzed the entropy of the 4 \glspl*{LSB} obtained from the \glspl*{IPI} from 42 subjects from mitdb and fantasia, and 111 subjects from BioSec\footnote{\url{https://www.comm.utoronto.ca/~biometrics/databases.html}} database. They claimed that the Shannon entropy was gradually decreasing when taking more significant bits. 

The same year, Altop \etal\ \cite{Altop2017} proposed a key generation protocol based on \glspl*{IPI}. Authors used to test their proposal 50 subjects from the MIMIC II Waveform \cite{mimic2}, and they calculated the Shannon entropy to check how entropic the heart signals are.  

A year later, in 2018, Sammoud \etal\ \cite{Sammoud2018} propose an \gls*{IPI}-based key distribution protocol where the keys are directly derived from the heart signal. In particular, there are three parties involved in the protocol, a central node in charge of providing the secure channel between the other (two) nodes who want to establish a secure channel between them. The main idea is that nodes share a secret key with that central node but they do not want to share it with the target node in such a way that they derive a new one from the heart signal. Finally, authors rely on a \gls*{BCH} to recover a similar key in both sensors.

Researchers demonstrated that the last 4 bits of the \glspl*{IPI} (positions 5678) have entropy \cite{Xu2011,Venkatasubramanian2010,Poon2006,Rostami2013}. However, Ortiz \etal\ \cite{Ortiz2020} carried out an in-depth analysis with more than 160,000 signals from over 20 datasets of the Physionet repository and used the NIST 800-90B recommendation to evaluate the tokens generated from different positions of the \glspl*{IPI}. In particular, they propose to use the combination of bits located in positions 2638 instead of the common assumed 5678. 

In addition to that, recently Ortiz \etal\ pointed out \cite{Ortiz2019} that using a \gls*{BCH} is not enough to recover the same token in different devices despite using the same signal. They demonstrated that a synchronization phase is a must to synchronize the signals before deriving the same token in different locations.



%\pica{Pirbhulal et al. [73] proposed a new biometric based algorithm for WBANs using HRV in key generation phase for making system secure and the proposed algorithm is compared with three other well known authentication methods use in WBAN are Rivest Shamir Adleman (RSA), Physiological Signal based Key Agreement (PSKA) and Data Encryption Standard (DES). Result shows that the proposed algorithm is more competent in terms of power utilization, transmission time utilization and average remaining energy. Previous protocols have similar objectives to H2H but they are facing a lot of serious issues which make them weak for deployment.}

%\pica{To overcome some of the serious limitations associated with previous H2H protocols, Rostami et al. [74] introduced lightweight heart-to-heart (H2H) authentication system for implanted medical sensors is utilizing heartbeats (ECG) data for key generation, key agreement and authentication is well suited for authentication to cardiac IMDs. The proposed protocol takes out time-varying arbitrariness from ECG signals and utilizes this arbitrariness to resist against many security attacks. This H2H authentication protocol is lightweight because it only needs a low-exponent RSA encryption and only few AES invocations and hash calculations by IMD.}

%\pica{Cho et al. [75] presented a lightweight key establishment protocol known as “Efficient Secret Key Delivery Using Heartbeats” is utilizing inter-pulse interval (IPI) of PPG physiological signals with the intention of eliminating demerits of the fuzzy vault protocol. The proposed protocol establishes a secret key using IPIs and it is shared between sender and receiver nodes. The proposed protocol is consisting of many phases: (i). witness generation (ii). ECC encoding and decoding (iii). Key generation (iv). Key transmission v. Key derivation (vi). Key verification and (vii). Key confirmation. The main advantage of the proposed protocol is reducing the key generation time by decreasing the length of witness and at the same time, it is preserving the benefits of the IPI based key establishment protocols. The proposed protocol supports basic prerequisite of the security of the medical services like treatment, diagnosis and prevention etc. Although some existing key establishment schemes are facing problems like high communication and computational costs for maintaining the network security but the proposed protocol is efficient as compare to previous protocols because it needs comparatively less time while maintaining good level of security.}


%\pica{Zaghouani et al. [18] proposed ECG based authentication scheme for e-healthcare system, it authenticates patient while protecting the privacy of the sending ECG signals. The proposed authentication scheme permits authentication node and the target application to make a secure authentication even though the authentication process is completed by using an untrusted channel. Finally, this scheme is using linear prediction code (LPC) to hide the important ECG data and this scheme emerges as a substitute to the fuzzy vault method.}

%\pica{Zebboudj et al. [80] presented competent and secure ECG based authentication system for e-healthcare system based on new biometric feature extraction mechanism which accomplishes higher proficiency of authentication amongst the sensor nodes. This scheme permits every pair of sensor nodes in the identical medical body area sensor networks (MBASNs) to share one secrete key that has been shared securely between them. In this proposed work, Elliptic-Curve Diffie-Hellman (ECDH) key agreement protocol is used to produce a common secrete key which not only guarantees encryption but at the same time, it also ensures the biometric based authentication of the sensor devices in the network. According to Sofia Zebboudj et al., the proposed authentication scheme feature extraction technique accomplishes superior performances as compare to the improved fast Fourier transform (FFT) technique because it reduces false acceptance rate (FAR), false recognition rate (FRR) and the period of time of the ECG signal.}

%\pica{Chen et al. [81] introduced finger ECG-based authentication scheme for healthcare using two-phases authentication utilizing artificial neural network (NN) models that balance the inaccurate performance of rejection and acceptance. In the first phase, a “General” NN model is created based on the data from the cohort and utilized it for first round screening and in the second phase, personal NN models are created from each particular user data as fine-grained recognition. The proposed algorithm allows very quick authentication by utilizing just 3 beats within 3 s. The proposed authentication algorithm is tested in a laboratory experiment with 50 subjects and result in average FRR and FAR under 10%. This performance will be more superior for less than 30 groups of cohort and result in average FRR and FAR below 5%. This algorithm is checked on the entire data set and various sizes of subsets containing 5, 10, 20, 30 and 40. From the results it is cleared that the introduced algorithm is trustworthy and very much realistic for user authentication and have average FRR and FAR under 10% for the entire data set.}

%\pica{PPG can be also used as authentication method instead of ECG in WBANs and PPG is quite uncomplicated non-persistent and inexpensive optical process use in authentication schemes. It could be also utilized to discover blood level varies on the micro vascular cot of individual tissue [82]. PPG signals are collected via attaching sensors to ear or finger and light is used to illuminate the body and observed blood flow in the user body. PPG signals are produced because of unintentional body processes and that is why it is impossible to be copied. The PPG signals might be utilized in healthcare system for a lot of reasons because they offers many benefits such as it may be utilized to measure blood pressure and oxygen etc. as compare to other type of biometric systems and due to these benefits, it is preferable approach for authentication schemes use in WBANs.}

%\pica{Recently, Reddy et al. [83] proposed enhanced biometric security system via two-level authentication based on PPG signals and PPG signals are collected via face and finger of the subject of cross-relationship. Finger print and face detection is carried out at first level, however, the security of both of them could be easily violated by using 3D printed finger tips or using face masking through surgery or through 3D printed face masks wearing. For these reasons, a second level security is required and therefore, proposed authentication scheme has utilized PPG signals to improve security.}

%\pica{Choudhary et al. [20] introduced authentication scheme for WBANs and mobile health applications is based on noise-robust PPG based biometric utilizing pulsatile waveform relationship. The introduced authentication scheme has four different phases and it is tested and validated utilizing PPG signal got from twenty-four real and six pretender subjects. The performance assessment outcomes illustrate that the proposed authentication scheme utilizing NCC metric get a FRR of 0.32 and FAR of 0.32 for the threshold of 0.997 and it means that the proposed authentication scheme is far better because it has lower computational cost as compare to other PPG based authentication schemes.}

%\pica{Karimian et al. [84] proposed non-fiducial PPG based authentication for healthcare system and the proposed work looks over non-fiducail characteristic extraction for PPG based authentication scheme for the first. In the proposed scheme, two steps feature selection procedure has been used which could result in a degree of freedom to eliminate the interrelated feature that may reduce authentication performance. In the first step, Kolmogorov-Smirnov (KS-test) is used to eliminate interrelated features because a feature will be judged superior if it is well interrelated to a class without any connection to other features and in the second step, Kemal PCA (KPCA) is a nonlinear method utilized for dimensionality decline and the authentication precision get better when dimensionality declines. Finally, supervised and unsupervised machine learning methods are used for authentication performance evolution. The performance outcome shows that 99.84% precision with EER of 1.31% could be attained based on non-fiducial extraction.}

==> sections/attacks.tex <==
\section{Attacks}\labe{sec:attacks}

Calleja \etal\ \cite{Calleja2015} could recover the \glspl*{IPI} of people by means of a web cam, being able to generate the same \glspl*{IPI} as on-body devices. Similar results were reported 3 years later by Seepers \etal\ \cite{Seepers2018}. 

Marin \etal\ \cite{Marin2016} by performing a reverse-engineering process and testing against 10 different \glspl*{IMD}, discovered that a weak adversary without being in direct contact with the device can perform a DoS attack and thus compromise the patient's safety. 

Marin \etal\ \cite{Marin2019} showed that both Biosec \cite{Cherukuri2003} and H2H \cite{Rostami2013} suffer from security pitfalls and give some guidelines to implement fuzzy extractors in a secure manner.

==> sections/new_bib.tex <==
\section{New found biblio}

Here we can cite new bib to add later  \cite{Cherukuri2003,Dodangeh2018,Belkhouja2019,Chizari2019}

%\pica{copied:} \say{With the emergence of new sensors, researchers started to investigate the feasibility of using these sensors to detect heartbeat signals. Lin et al. \cite{Lin2019} proposed the first piezoelectric sensor-based key generation system H2B for on-body wearable and implantable devices. H2B is based on the observation that the minor vibrations caused by heartbeats can be detected by piezoelectric sensors on different body locations. The evaluation results showed that H2B can pair two wearable devices on the same user’s body with a success rate of 95.6\%. Security analysis of H2B also demonstrated that it is secure against passive attack, active presentation attack and active video attack.}


%\begin{figure*}
%\centering
%\includegraphics[width=\textwidth]{figures/survey_IPI}
%\caption{Timeline of surveyed works.}
%\label{figure:survey_timeline}
%\end{figure*}

On going: \cite{Pirbhulal2018}

Already checked all works that reference \cite{Koya2018,Mahendran2020,Marin2019,Moosavi2017,Moosavi2017b,Reshan2019,Rostami2013,Seepers2014,Seepers2015,Sun2017,Wu2018,Zhang2012,Zheng2015,Zheng2019} in Scholar

==> sections/security.tex <==
\section{Security}\label{sec:security}
\lara{intro}


